Understanding the Generalization Benefit of Model Invariance from a Data Perspective

Machine learning models that are developed with invariance to certain types of data transformations have demonstrated superior generalization performance in practice. However, the underlying mechanism that explains why invariance leads to better generalization is not well-understood, limiting our ability to select appropriate data transformations for a given dataset. This paper studies the generalization benefit of model invariance by introducing the sample cover induced by transformations, i.e., a representative subset of a dataset that can approximately recover the whole dataset using transformations. Based on this notion, we refine the generalization bound for invariant models and characterize the suitability of a set of data transformations by the sample covering number induced by transformations, i.e., the smallest size of its induced sample covers. We show that the generalization bound can be tightened for suitable transformations that have a small sample covering number. Moreover, our proposed sample covering number can be empirically evaluated, providing a practical guide for selecting transformations to develop model invariance for better generalization. We evaluate the sample covering numbers for commonly used transformations on multiple datasets and demonstrate that the smaller sample covering number for a set of transformations indicates a smaller gap between the test and training error for invariant models, thus validating our propositions.

==> _checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~?.} %\ref{gen_inst}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> include/supp_macros.tex <==
\newcommand*{\mytensor}[1]{\bm{\mathcal{#1}}}
\newcommand*{\mymatrix}[1]{\bm{#1}}
\newcommand*{\myvector}[1]{\bm{#1}}
\newcommand*{\noise}[1]{\widehat{#1}}
\newcommand*{\mm}{\mymatrix}
\newcommand*{\mv}{\myvector}
\newcommand{\mt}{\mytensor}
\newcommand*{\mmCols}[2]{\mm{#1}_{[#2]}}

% names
\newcommand{\modname}{{TempLe}\xspace}
\newcommand{\modnamefull}{{Template Learning}\xspace}
\newcommand{\ourmod}{{O-TempLe}\xspace}
\newcommand{\ourmodfull}{{Online Template Learning}\xspace}
\newcommand{\ourmodtwo}{{FM-TempLe}\xspace}
\newcommand{\ourmodtwofull}{{Finite-Model Template Learning}\xspace}
\newcommand{\patnamefull}{{Transition Template}\xspace}
\newcommand{\patnamefulls}{{Transition Templates}\xspace}
\newcommand{\patnamelowercase}{{transition template}\xspace}
\newcommand{\patname}{\textsf{TT}\xspace}
\newcommand{\patnames}{\textsf{TT}s\xspace}
\newcommand{\patfunc}{{Templatize}\xspace}
\newcommand{\probgapname}{{ranking gap}\xspace}

% notations
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\pattern}{\mathbf{g}}
\newcommand{\patp}{\mathbf{g}^{(p)}}
\newcommand{\patr}{g^{(r)}}
\newcommand{\patsp}{g^{(p)}}
\newcommand{\pats}{g}
\newcommand{\patset}{\mathcal{G}}
\newcommand{\patvisset}{\mathcal{O}}
\newcommand{\patvis}{\mathbf{o}}
\newcommand{\patvisp}{\mathbf{o}^{(N)}}
\newcommand{\patvisr}{o^{(R)}}
\newcommand{\mdpset}{\mathcal{C}}
\newcommand{\permut}{\mathbf{\sigma}}
\newcommand{\dist}{\rho}
\newcommand{\thressm}{m_s}
\newcommand{\threslg}{m}
\newcommand{\mingap}{\omega}
\newcommand{\kset}{\mathcal{K}}

% algorithm2e
% \SetKwInput{Input}{Input}
% \SetKwInput{Output}{Output}
% \SetKwInput{Parameter}{Parameters}
% \SetKwFunction{Up}{Update}
% \SetKwFunction{Sin}{SingleRMax}
% \SetKwFunction{Pa}{Patternize}
% \SetKwProg{Fn}{Function}{:}{}

%algorithmic
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
% \floatname{algorithm}{Algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% previous
\newcommand{\dmname}{{dynamic matrix}\xspace}
\newcommand{\dmnames}{{dynamic matrices}\xspace}
\newcommand{\avgrew}{{AvgReward}\xspace}
\newcommand{\pavgrew}{{PostAvgReward}\xspace}
\newcommand{\numepi}{{TotalEps}\xspace}
\newcommand{\walkname}{{$\beta$-curious walking}\xspace}

%\newcommand{\noisebound}{\mathsf{gap}}
\newcommand{\coherence}{c_{\mathsf{max}}}
\newcommand{\gap}{\mathsf{gap}}
\newcommand{\op}{\mathsf{op}}
\newcommand{\diag}{\mathsf{Diag}}
\newcommand{\identity}{\mathbf{\mathds{1}}}
\newcommand{\identitymatrix}{\mm{I}}
\newcommand\R{\mathbb{R}}
\newcommand\BlkDiagFFT{\mathbf{\Theta}}
\newcommand\SuperLong{\mathsf{\sigma}}
\newcommand\defeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}
\newcommand\CirOneD{\mathsf{Cir_{1\!-\!d}}}
\newcommand\CirTwoD{\mathsf{Cir_{2\!-\!d}}}
\newcommand\DFTOneD{\mathsf{DFT_{1\!-\!d}}}
\newcommand\DFTTwoD{\mathsf{DFT_{2\!-\!d}}}
\newcommand\vectorize{\mathsf{flat}}
\newcommand{\Mod}[1]{\ (\text{mod}\ #1)}
\newcommand\CCir{\mathsf{Blk}\CirTwoD}

\def\viz{{viz.,\ \/}}
\newcommand{\suchthat}{\, \mid \,}
\def\Pbb{{\mathbb P}}
\def\Rbb{\mathbb{R}}
\def\Ebb{\mathbb{E}}
\def\tha{{\mbox{\tiny th}}}
\def\beq{\begin{equation}}
\def\bfI{{\mathbf I}}
\def\nn{\nonumber}
\def\eeq{\end{equation}\noindent}
\def\ci{\perp\!\!\!\perp} % from Wikipedia
\def\bfU{{\mathbf U}}
\newcommand{\redt}{\textcolor[rgb]{1,0,0}}
\newcommand{\bluet}{\textcolor[rgb]{0,0,1}}
\newcommand{\greent}{\textcolor[rgb]{0,1,0}}
\newcommand*{\conj}[1]{\overline{#1}}
\newcommand*{\hermconj}{^{\mathsf{H}}}


%\newcommand{\bp}{\begin{psfrags}}
%\newcommand{\ep}{\end{psfrags}}
%\newcommand{\bc}{\begin{center}}
%\newcommand{\ec}{\end{center}}

\newcommand{\llvert}{\left\vert\vphantom{\frac{1}{1}}\right.}
\newcommand{\xcmd}[2]{\left(#1\,\left\vert\vphantom{#1#2}\right. #2\right)}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand*{\tcr}[1]{\textcolor{red}{#1}}
\newcommand*{\tcb}[1]{\textcolor{blue}{#1}}
\newcommand*{\textcal}[1]{%
  % family qzc: Font TeX Gyre Chorus (package tgchorus)
  % family pzc: Font Zapf Chancery (package chancery)
  \textit{\fontfamily{qzc}\selectfont#1}%
}
\newcommand{\shift}{\mathsf{Shift}}
\newcommand{\circshift}{\mathsf{Circshift}}
\newcommand{\ranktest}{\mathsf{RankTest}}
\newcommand{\sentence}{P}
\newcommand{\patch}{\mathcal{P}}

\newcommand{\Conv}{\mathop{\scalebox{1.5}{\raisebox{-0.2ex}{$\ast$}}}}%
\newcommand{\Toep}{\mathsf{Cir}}
\newcommand{\Cir}{\mathsf{Cir}}
\newcommand{\BCir}{\mathsf{BlkCir}}
\newcommand{\CToep}{{\mathcal{F}}}
%\newcommand{\CCir}{{\mathcal{F}}}
\newcommand{\Diag}{\mathsf{Diag}}
\newcommand{\Pair}{\mathsf{Pair}}
\newcommand{\Trip}{\mathsf{Trip}}
\newcommand{\Rank}{\mathsf{Rank}}
\newcommand{\DFT}{\mathsf{FFT}}

\newcommand*{\tran}{^{\mkern-1.5mu\mathsf{T}}}


\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\fro}{\mathsf{F}}
\DeclareMathOperator{\flatten}{unfold}
\DeclareMathOperator{\modeA}{\mathcal{F}}
\DeclareMathOperator{\modeB}{\mathcal{G}}
\DeclareMathOperator{\modeC}{\mathcal{H}}

\DeclareMathOperator{\basisV}{V_{basis}}

\DeclareMathOperator{\stationaryV}{v}
\DeclareMathOperator{\basis}{b}
\DeclareMathOperator{\coeff}{c}
\DeclareMathOperator{\errorTensor}{\mathcal{E}}
\DeclareMathOperator{\Cum}{C_3}
\DeclareMathOperator{\mat}{mat}
\DeclareMathOperator{\newCum}{M}
\DeclareMathOperator{\Fbb}{\mathbb{F}}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\block}{blk}
\DeclareMathOperator{\blkdiag}{Blkdiag}
\DeclareMathOperator{\Tr}{\mathsf{trace}}
\DeclareMathOperator{\poly}{poly}
\def\calT{{\mathcal{ T}}}
%\newcommand{\fix}{\marginpar{FIX}}
%\newcommand{\new}{\marginpar{NEW}}
%%%%%%%%% new theoretical guaranteed symbols %%%%%%%%%%
\DeclareMathOperator{\onefilter}{f}
\DeclareMathOperator{\cirf}{\mathcal{F}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{property}[theorem]{Property}
\newtheorem{condition}{Condition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{myfact}{Fact}
\newtheorem{assumption}{Assumption}
\floatname{algorithm}{Algorithm}
%\renewcommand{\algorithmicxrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicxensure}{\textbf{Output:}}
% \makeatletter
% \def\thm@space@setup{%
%   \thm@preskip=0.3em
%   \thm@postskip=0.2em % or whatever, if you don't want them to be equal
% }
% \makeatother

\newcommand\FFTratio{\mathbf{\Gamma}}

\newcommand{\yc}{\textcolor[rgb]{0,0,1}{YC: }\textcolor[rgb]{0,0,1}}
\newcommand{\fh}[1]{\textcolor[rgb]{1,0,0}{[FH: #1]}} 
\colorlet{soulcyan}{cyan!30}
\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{soulcyan}\hl{#1}}}

==> include/supp_packages.tex <==
\usepackage{url}
\usepackage{dsfont}
\usepackage{xspace}
%\usepackage{hyperref}
%\usepackage{times}
% \usepackage[authoryear]{natbib}
% \usepackage[square,sort,comma,numbers]{natbib}
% \usepackage{natbib}
\usepackage[outdir=./]{epstopdf}
\usepackage{graphicx,float,pgfplots,wrapfig,sidecap,lipsum}
\usepackage{booktabs}
\usepackage{paralist}

\usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{algpseudocode}
% \newcommand{\theHalgorithm}{\arabic{algorithm}}
% \usepackage[linesnumbered,algoruled,boxed,lined]{algorithm2e}
% \usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
%\usepackage[pass]{geometry}
\usepackage{amsfonts}
\usepackage{lipsum}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage{xcolor}
\usepackage[font=normal,labelfont=bf]{caption}
\usepackage{mathtools} 
\usepackage{bbm}
\usepackage{multirow}
\usepackage{comment}

\usepackage{tablefootnote}
%\usepackage{subfig}
\usepackage{subcaption}
\usepackage{subfloat}
% \usepackage{hyperref,psfrag} % not allowed by AAAI
\usepackage{tikz}
\usetikzlibrary{fit}
\usetikzlibrary{calc,shapes}
\usetikzlibrary{decorations.pathmorphing} % noisy shapes
\usetikzlibrary{fit}					% fitting shapes to coordinates
\usetikzlibrary{backgrounds}	% drawing the background after the foreground

% \usepackage{refcheck}

\usepackage{bm}
\usepackage{mathrsfs} 
%\usepackage{fourier}
\usepackage{stmaryrd}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{diagbox}

%pgfplots
\usepackage[utf8]{inputenc}
% \usepackage{fontspec}  % optional
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{dateplot}
\usepackage{soul}


